Grounding Multilingual Multimodal LLMs With Cultural Knowledge

Multimodal Large Language Models excel in high-resource settings, but often misinterpret long-tail cultural entities and underperform in low-resource languages. To address this gap, we propose a data-centric approach that directly grounds MLLMs in cultural knowledge. Leveraging a large scale knowledge graph from Wikidata, we collect images that represent culturally significant entities, and generate synthetic multilingual visual question answering data. The resulting dataset, CulturalGround, comprises 22 million high-quality, culturally-rich VQA pairs spanning 42 countries and 39 languages. We train an open-source MLLM CulturalPangea on CulturalGround, interleaving standard multilingual instruction-tuning data to preserve general abilities. CulturalPangea achieves state-of-the-art performance among open models on various culture-focused multilingual multimodal benchmarks, outperforming prior models by an average of 5.0 without degrading results on mainstream vision-language tasks. Our findings show that our targeted, culturally grounded approach could substantially narrow the cultural gap in MLLMs and offer a practical path towards globally inclusive multimodal systems.

==> latex/tables/evals.tex <==
\begin{table}[t]
  \centering
  \footnotesize
  \begin{tabular}{@{}lcccl@{}}
    \toprule
    \textbf{Benchmark} 
      & \textbf{\# L} 
      & \textbf{Samples} 
      & \textbf{Type} 
      & \textbf{Metric} \\
    \midrule
    CVQA (Local) & 28 & 10K & MC & Exact-match \\
    MaRVL & 5 & 6K & OE & Exact-match \\
    XM100 & 36 & 3.6K & OE & CIDER \\
    ALM-Bench & 39 & 1.3K & Mixed & LLM-Judge \\
    MERLIN & 5 & 7K & OE & Exact-match \\
    MaXM & 6 & 2K & OE & Relaxed Acc. \\
    M3Exam & 6 & 3K & MC & Exact-match \\
    \bottomrule
  \end{tabular}
  \caption{Overview of multilingual multimodal benchmarks} %"Samples" denotes the approximate number of questions or captions; "Q Type" is whether items are multiple‐choice (MC), open‐ended (OE), or mixed; "Metric" is the evaluation protocol.}
  \label{tab:benchmarks_overview}
\end{table}

==> latex/tables/merlin.tex <==
% \subsection{MERLIN}
% We show the performance of different models on the MERLIN benchmark in \autoref{tab:breakdown:merlin}.
% \begin{table*}[t]
% \centering
% \small
% \begin{tabular}{@{}l|cccccc@{}}
% \toprule
% \textbf{Model}        & \textbf{Multi} & \textbf{Hindi} & \textbf{Tamil} & \textbf{Indonesian} & \textbf{Japanese} & \textbf{Vietnamese} \\
% \midrule
% Llava-Next-7B         & 34.1 & 30.1 & 13.0 & 42.4 & 41.9 & 43.1 \\
% Molmo-7B-D            & 42.9 & 30.8 & 15.8 & 54.7 & 53.8 & 59.5 \\
% Llama3.2-11B          & 49.1 & 60.6 &  2.4 & 64.6 & 55.1 & 62.6 \\
% PaliGemma-3B          & 13.1 & 12.6 &  2.5 & 22.0 & 13.7 & 15.0 \\
% mBLIP mT0-XL          & 15.8 & 10.8 & 11.0 & 19.2 & 14.9 & 23.3 \\
% AyaVision-8B          & 55.3 & 55.5 & 40.5 & 55.3 & 62.6 & 62.9 \\
% Pangea-7B             & 66.0 & 64.6 & 50.2 & 66.7 & 74.1 & 74.3 \\
% \model      & 81.1 & 77.0 & 76.2 & 80.6 & 85.8 & 85.7 \\
% \bottomrule
% \end{tabular}
% \caption{Performance of selected models on the MERLIN across different languages.}
% \label{tab:breakdown:merlin}
% \end{table*}


==> latex/tables/new_data_table_all_regions.tex <==
% \begin{table*}[t]
%   \centering
%   \small
%   \begin{tabular}{lrrrrrrrrr}
%     \toprule
%     \multirow{2}{*}{\textbf{Regions}} & \multirow{2}{*}{\textbf{Images}} & \multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}r@{}}Unique\\Entities\end{tabular}}} & \multicolumn{6}{c}{\textbf{Languages}} & \multirow{2}{*}{\textbf{Total}} \\
%     \cmidrule(lr){4-9}
%     & & & \textbf{vi} & \textbf{id} & \textbf{ta} & \textbf{hi} & \textbf{ja} & \textbf{en} & \\
%     \midrule
%     Vietnam & 17,554 & 4,798 & 15,007 & 4,813 & 2,731 & 2,897 & 7,632 & 15,829 & 48,909 \\
%     Indonesia & 41,350 & 20,820 & 12,143 & 45,357 & 9,070 & 9,424 & 16,561 & 45,336 & 137,891 \\
%     Japan & 313,743 & 135,593 & 96,646 & 119,289 & 71,554 & 76,245 & 415,290 & 389,397 & 1,168,421 \\
%     India & 147,871 & 48,405 & 116,652 & 127,477 & 152,707 & 162,787 & 133,184 & 234,996 & 927,803 \\
%     \midrule
%     All Regions & 520,518 & 209,616 & 240,448 & 296,936 & 236,062 & 251,353 & 572,667 & 685,558 & 2,283,024 \\
%     \bottomrule
%   \end{tabular}
%         \caption{CulturalGround dataset statistics showing the distribution of images, unique entities, and multilingual VQA samples across target languages (Vietnamese, Indonesian, Tamil, Hindi, Japanese, English) for each major cultural region in our study.}
%         \label{tab:wikidata_stats}
% \end{table*}


% \begin{table*}[t]
%   \centering
%   \scriptsize
%   \setlength{\tabcolsep}{3pt}
%   \resizebox{\textwidth}{!}{%
%   \begin{tabular}{l*{12}{r}}
%     \toprule
%     \multirow{2}{*}{\textbf{Region}} &
%     \multicolumn{7}{c}{\textbf{Raw Data}} &
%     \multicolumn{2}{c}{\textbf{Region Sampling}} &
%     \multicolumn{2}{c}{\textbf{Language Sampling}} &
%     \multirow{2}{*}{\textbf{Total}} \\
%     \cmidrule(lr){2-8} \cmidrule(lr){9-10} \cmidrule(lr){11-12}
%     & \textbf{Entities} & \textbf{Images} & \textbf{Templates VQA} & \textbf{Q/Entity}
%     & \textbf{OE Reph.} & \textbf{MCQs} & \textbf{Overall}
%     & \textbf{OE} & \textbf{MCQs}
%     & \textbf{OE} & \textbf{MCQs} & \\
%     \midrule
%     Germany        & 562\,945  & 350\,828  & 2\,752\,049 & 4.9 & 2\,752\,048 & 1\,375\,424 & 2\,836\,115 & 931\,184 & 346\,667 & 922\,583 & 343\,159 & 1\,265\,742 \\
%     France         & 401\,170  & 276\,983  & 2\,676\,840 & 6.7 & 2\,676\,838 & 1\,338\,354 & 2\,730\,428 & 922\,385 & 344\,505 & 915\,237 & 341\,454 & 1\,256\,691 \\
%     United Kingdom & 323\,665  & 328\,906  & 1\,355\,580 & 4.2 & 1\,355\,577 &   677\,746 & 2\,184\,596 & 872\,363 & 339\,909 & 866\,450 & 338\,013 & 1\,204\,463 \\
%     Czechia        & 210\,282  & 198\,223  &   636\,978 & 3.0 &   636\,978 &   318\,396 &   994\,894 & 716\,636 & 278\,443 & 647\,893 & 256\,139 &   904\,032 \\
%     % … repeat for the remaining regions … 
%     \midrule
%     \textbf{Total} & 3\,044\,895 & 2\,879\,840 & 15\,872\,010 & 6.6 & 15\,871\,990 & 4\,757\,103 & 21\,986\,501 & 14\,105\,480 & 5\,457\,881 & 12\,884\,568 & 5\,021\,871 & 17\,906\,439 \\
%     \bottomrule
%   \end{tabular}%
%   }
%   \caption{Per-region counts: raw VQA templates, per-entity ratio, post-rephrasing open-ended VQA, MCQs, and “overall” after region- and language-level sampling.}
%   \label{tab:region_data_styled}
% \end{table*}

% \begin{table*}[t]
%   \centering
%   \scriptsize
%   \setlength{\tabcolsep}{3pt}
%   \resizebox{\textwidth}{!}{%
%   \begin{tabular}{l*{12}{r}}
%     \toprule
%     \multirow{2}{*}{\textbf{Region}} &
%     \multicolumn{7}{c}{\textbf{Raw Data}} &
%     \multicolumn{2}{c}{\textbf{Region Sampling}} &
%     \multicolumn{2}{c}{\textbf{Language Sampling}} &
%     \multirow{2}{*}{\textbf{Total}} \\
%     \cmidrule(lr){2-8} \cmidrule(lr){9-10} \cmidrule(lr){11-12}
%     & \textbf{Entities} & \textbf{Images} & \textbf{Templates VQA} & \textbf{Q/Entity}
%     & \textbf{OE Reph.} & \textbf{MCQs} & \textbf{Overall}
%     & \textbf{OE} & \textbf{MCQs}
%     & \textbf{OE} & \textbf{MCQs} & \\
%     \midrule
%     Germany        & 562\,945  & 350\,828  & 2\,752\,049 & 4.9 & 2\,752\,048 & 1\,375\,424 & 2\,836\,115 & 931\,184 & 346\,667 & 922\,583 & 343\,159 & 1\,265\,742 \\
%     France         & 401\,170  & 276\,983  & 2\,676\,840 & 6.7 & 2\,676\,838 & 1\,338\,354 & 2\,730\,428 & 922\,385 & 344\,505 & 915\,237 & 341\,454 & 1\,256\,691 \\
%     United Kingdom & 323\,665  & 328\,906  & 1\,355\,580 & 4.2 & 1\,355\,577 &   677\,746 & 2\,184\,596 & 872\,363 & 339\,909 & 866\,450 & 338\,013 & 1\,204\,463 \\
%     Czechia        & 210\,282  & 198\,223  &   636\,978 & 3.0 &   636\,978 &   318\,396 &   994\,894 & 716\,636 & 278\,443 & 647\,893 & 256\,139 &   904\,032 \\
%     Spain          & 195\,481  & 216\,019  &   985\,241 & 5.0 &   985\,241 &   492\,606 & 1\,522\,659 & 797\,086 & 310\,035 & 775\,047 & 302\,656 & 1\,077\,703 \\
%     Italy          & 179\,948  & 222\,351  & 1\,133\,463 & 6.3 & 1\,133\,463 &   566\,713 & 1\,764\,383 & 826\,994 & 325\,167 & 814\,214 & 320\,792 & 1\,135\,006 \\
%     Poland         & 163\,502  & 131\,155  &   753\,751 & 4.6 &   753\,750 &   376\,863 &   936\,987 & 705\,972 & 271\,105 & 654\,479 & 252\,401 &   906\,880 \\
%     Russia         & 160\,695  & 180\,253  &   613\,822 & 3.8 &   613\,822 &   306\,698 &   848\,805 & 688\,741 & 267\,857 & 623\,098 & 245\,876 &   868\,974 \\
%     Japan          & 140\,966  & 145\,843  &   793\,762 & 5.6 &   793\,759 &   396\,870 & 1\,215\,080 & 753\,365 & 291\,601 & 725\,737 & 282\,833 & 1\,008\,570 \\
%     Netherlands    & 129\,687  &  72\,709  &   375\,078 & 2.9 &   375\,078 &   187\,379 &   375\,078 & 375\,078 &  75\,303 & 287\,443 &  34\,386 &   321\,289 \\
%     Ukraine        &  90\,165  & 100\,367  &   367\,819 & 4.1 &   367\,819 &   183\,731 &   562\,820 & 562\,820 &  73\,816 & 466\,063 & 185\,818 &   651\,881 \\
%     Brazil         &  67\,632  &  68\,775  &   419\,684 & 6.2 &   419\,684 &   209\,577 &   648\,573 & 643\,938 &  84\,099 & 552\,964 & 218\,144 &   771\,108 \\
%     China          &  52\,862  &  68\,858  &   288\,525 & 5.5 &   288\,524 &   144\,258 &   469\,809 & 469\,809 &  20\,129 & 396\,508 & 170\,069 &   565\,677 \\
%     India          &  50\,974  &  72\,683  &   365\,804 & 7.2 &   365\,804 &   182\,549 &   717\,590 & 660\,425 &  25\,784 & 601\,327 & 239\,121 &   840\,448 \\
%     Norway         &  45\,376  &  47\,615  &   255\,226 & 5.6 &   255\,226 &   127\,609 &   382\,293 & 382\,293 &  51\,068 & 322\,590 & 124\,876 &   474\,466 \\
%     Portugal       &  28\,521  &  35\,229  &   155\,542 & 5.5 &   155\,542 &    77\,735 &   237\,215 & 237\,215 &  31\,154 & 199\,808 &  79\,212 &   279\,020 \\
%     Israel         &  27\,592  &  33\,731  &   183\,099 & 6.6 &   183\,099 &    91\,493 &   290\,266 & 290\,266 &  36\,557 & 251\,987 & 109\,146 &   361\,133 \\
%     Romania        &  25\,571  &  26\,451  &   196\,705 & 7.7 &   196\,705 &    98\,302 &   287\,167 & 287\,167 &  39\,296 & 253\,683 &  96\,749 &   350\,432 \\
%     Indonesia      &  22\,249  &  22\,060  &   145\,834 & 6.6 &   145\,832 &    72\,817 &   257\,405 & 257\,405 &  28\,964 & 222\,554 &  79\,919 &   302\,473 \\
%     Turkey         &  19\,470  &  23\,876  &   163\,963 & 8.4 &   163\,963 &    81\,913 &   256\,861 & 256\,861 &  32\,509 & 225\,631 &  94\,869 &   320\,500 \\
%     South Korea    &  18\,995  &  15\,175  &   149\,796 & 7.9 &   149\,796 &    74\,793 &   210\,015 & 210\,015 &  29\,782 & 183\,931 &  62\,974 &   246\,905 \\
%     Iran           &  18\,609  &  32\,496  &   114\,996 & 6.2 &   114\,996 &    57\,424 &   252\,436 & 252\,436 &  22\,938 & 217\,157 &  96\,251 &   313\,408 \\
%     Greece         &  18\,337  &  24\,887  &   125\,163 & 6.8 &   125\,163 &    62\,537 &   250\,587 & 250\,587 &  25\,017 & 219\,711 &  92\,265 &   311\,976 \\
%     Taiwan         &  16\,363  &  33\,410  &    71\,483 & 4.4 &    71\,483 &    35\,692 &   166\,461 & 166\,461 &  14\,390 & 136\,394 &  62\,726 &   199\,120 \\
%     Ireland        &  14\,302  &  22\,856  &    86\,838 & 6.1 &    86\,838 &    43\,359 &   185\,155 & 185\,155 &  17\,380 & 160\,854 &  70\,021 &   230\,875 \\
%     Bulgaria       &  13\,847  &  17\,315  &    94\,452 & 6.8 &    94\,452 &    47\,205 &   178\,002 & 178\,002 &  19\,012 & 158\,160 &  63\,677 &   221\,837 \\
%     Thailand       &   8\,983  &  15\,037  &    58\,398 & 6.5 &    58\,398 &    29\,140 &   125\,405 & 125\,405 &  11\,512 & 108\,555 &  47\,116 &   155\,671 \\
%     Nigeria        &   6\,073  &   6\,368  &    42\,080 & 6.9 &    42\,080 &    21\,017 &    77\,514 & 77\,514 &   8\,352 &  67\,735 &  25\,967 &    93\,702 \\
%     Malaysia       &   6\,008  &   9\,788  &    38\,208 & 6.4 &    38\,208 &    19\,058 &    80\,754 & 80\,754 &   7\,516 &  69\,137 &  29\,487 &    98\,624 \\
%     Vietnam        &   5\,048  &   5\,744  &    37\,035 & 7.3 &    37\,035 &    18\,492 &    58\,661 & 58\,661 &   7\,345 &  50\,720 &  21\,135 &    71\,855 \\
%     Bangladesh     &   5\,023  &   9\,236  &    29\,253 & 5.8 &    29\,253 &    14\,599 &    62\,839 & 62\,839 &   5\,768 &  53\,756 &  23\,890 &    77\,646 \\
%     Pakistan       &   4\,761  &   6\,973  &    38\,006 & 8.0 &    38\,005 &    18\,961 &    77\,271 & 77\,271 &   7\,516 &  68\,913 &  29\,338 &    98\,251 \\
%     Sri Lanka      &   1\,977  &   2\,651  &    14\,643 & 7.4 &    14\,643 &     7\,306 &    29\,512 & 29\,512 &   2\,857 &  26\,199 &  10\,929 &    37\,128 \\
%     Saudi Arabia   &   1\,874  &   2\,292  &    17\,759 & 9.5 &    17\,759 &     8\,868 &    35\,921 & 35\,921 &   3\,547 &  31\,957 &  13\,352 &    45\,309 \\
%     Kenya          &   1\,769  &   2\,763  &    17\,251 & 9.8 &    17\,251 &     8\,610 &    36\,397 & 36\,397 &   3\,537 &  32\,290 &  14\,015 &    46\,305 \\
%     Ethiopia       &   1\,399  &   2\,163  &    14\,244 &10.2 &    14\,244 &     7\,112 &    30\,317 & 30\,317 &   2\,920 &  27\,032 &  11\,759 &    38\,791 \\
%     Mongolia       &   1\,032  &   1\,306  &    12\,482 &12.1 &    12\,482 &     6\,237 &    23\,611 & 23\,611 &   2\,452 &  21\,413 &   8\,499 &    29\,912 \\
%     Tanzania       &     969  &   1\,454  &    11\,966 &12.3 &    11\,966 &     5\,983 &    26\,440 & 26\,440 &   2\,406 &  23\,693 &  10\,567 &    34\,260 \\
%     Rwanda         &     773  &   1\,393  &     7\,333 & 9.5 &     7\,332 &     3\,665 &    15\,711 & 15\,711 &   1\,469 &  13\,820 &   6\,157 &    19\,977 \\
%     Mexico         &  20\,622  &  29\,724  &   184\,998 & 9.0 &   184\,998 &    92\,497 &   363\,479 & 363\,479 &  37\,179 & 318\,079 & 132\,417 &   450\,496 \\
%     Egypt          &   6\,561  &   9\,596  &    63\,237 & 9.6 &    63\,237 &    31\,616 &   131\,069 & 131\,069 &  12\,692 & 120\,625 &  52\,695 &   173\,320 \\
%     Singapore      &   2\,589  &   4\,298  &    23\,624 & 9.1 &    23\,619 &    11\,811 &    49\,920 & 49\,920 &   4\,858 &  49\,141 &  21\,002 &    70\,143 \\
%     \midrule
%     \textbf{Total} & 3\,044\,895 & 2\,879\,840 & 15\,872\,010 & 6.6 & 15\,871\,990 & 7\,933\,015 & 21\,986\,501 & 14\,105\,480 & 5\,457\,881 & 12\,884\,568 & 5\,021\,871 & 17\,906\,439 \\
%     \bottomrule
%   \end{tabular}%
%   }
%   \caption{Per-region counts: raw VQA templates, per-entity ratio, post-rephrasing open-ended VQA, MCQs, and overall volumes after region- and language-level sampling.}
%   \label{tab:region_data_full_all}
% \end{table*}


% \begin{table*}[t]
%   \centering
%   \scriptsize
%   \setlength{\tabcolsep}{3pt}
%   \resizebox{\textwidth}{!}{%
%   \begin{tabular}{l*{8}{r}}
%     \toprule
%     \multirow{2}{*}{\textbf{Region}} & \multicolumn{5}{c}{\textbf{Raw Data}} & \multicolumn{2}{c}{\textbf{Region Sampling}} & \multirow{2}{*}{\textbf{Total}} \\
%     \cmidrule(lr){2-6} \cmidrule(lr){7-8}
%     & \textbf{Entities} & \textbf{Images} & \textbf{OE} & \textbf{MCQs} & \textbf{Overall} & \textbf{OE} & \textbf{MCQs} & 
%     \\
%     \midrule
%     Germany & 562\,945 & 350\,828 & 2\,752\,048 & 1\,375\,424 & 2\,836\,115 & 931\,184 & 346\,667 & 1\,265\,742 \\
%     France & 401\,170 & 276\,983 & 2\,676\,838 & 1\,338\,354 & 2\,730\,428 & 922\,385 & 344\,505 & 1\,256\,691 \\
%     United Kingdom & 323\,665 & 328\,906 & 1\,355\,577 & 677\,746 & 2\,184\,596 & 872\,363 & 339\,909 & 1\,204\,463 \\
%     Czechia & 210\,282 & 198\,223 & 636\,978 & 318\,396 & 994\,894 & 716\,636 & 278\,443 & 904\,032 \\
%     Spain & 195\,481 & 216\,019 & 985\,241 & 492\,606 & 1\,522\,659 & 797\,086 & 310\,035 & 1\,077\,703 \\
%     Italy & 179\,948 & 222\,351 & 1\,133\,463 & 566\,713 & 1\,764\,383 & 826\,994 & 325\,167 & 1\,135\,006 \\
%     Poland & 163\,502 & 131\,155 & 753\,750 & 376\,863 & 936\,987 & 705\,972 & 271\,105 & 906\,880 \\
%     Russia & 160\,695 & 180\,253 & 613\,822 & 306\,698 & 848\,805 & 688\,741 & 267\,857 & 868\,974 \\
%     Japan & 140\,966 & 145\,843 & 793\,759 & 396\,870 & 1\,215\,080 & 753\,365 & 291\,601 & 1\,008\,570 \\
%     Netherlands & 129\,687 & 72\,709 & 375\,078 & 187\,379 & 375\,078 & 375\,078 & 75\,303 & 321\,289 \\
%     Ukraine & 90\,165 & 100\,367 & 367\,819 & 183\,731 & 562\,820 & 562\,820 & 73\,816 & 651\,881 \\
%     Brazil & 67\,632 & 68\,775 & 419\,684 & 209\,577 & 648\,573 & 643\,938 & 84\,099 & 771\,108 \\
%     China & 52\,862 & 68\,858 & 288\,524 & 144\,258 & 469\,809 & 469\,809 & 20\,129 & 565\,677 \\
%     India & 50\,974 & 72\,683 & 365\,804 & 182\,549 & 717\,590 & 660\,425 & 25\,784 & 840\,448 \\
%     Norway & 45\,376 & 47\,615 & 255\,226 & 127\,609 & 382\,293 & 382\,293 & 51\,068 & 474\,466 \\
%     Portugal & 28\,521 & 35\,229 & 155\,542 & 77\,735 & 237\,215 & 237\,215 & 31\,154 & 279\,020 \\
%     Israel & 27\,592 & 33\,731 & 183\,099 & 91\,493 & 290\,266 & 290\,266 & 36\,557 & 361\,133 \\
%     Romania & 25\,571 & 26\,451 & 196\,705 & 98\,302 & 287\,167 & 287\,167 & 39\,296 & 350\,432 \\
%     Indonesia & 22\,249 & 22\,060 & 145\,832 & 72\,817 & 257\,405 & 257\,405 & 28\,964 & 302\,473 \\
%     Turkey & 19\,470 & 23\,876 & 163\,963 & 81\,913 & 256\,861 & 256\,861 & 32\,509 & 320\,500 \\
%     South Korea & 18\,995 & 15\,175 & 149\,796 & 74\,793 & 210\,015 & 210\,015 & 29\,782 & 246\,905 \\
%     Iran & 18\,609 & 32\,496 & 114\,996 & 57\,424 & 252\,436 & 252\,436 & 22\,938 & 313\,408 \\
%     Greece & 18\,337 & 24\,887 & 125\,163 & 62\,537 & 250\,587 & 250\,587 & 25\,017 & 311\,976 \\
%     Taiwan & 16\,363 & 33\,410 & 71\,483 & 35\,692 & 166\,461 & 166\,461 & 14\,390 & 199\,120 \\
%     Ireland & 14\,302 & 22\,856 & 86\,838 & 43\,359 & 185\,155 & 185\,155 & 17\,380 & 230\,875 \\
%     Bulgaria & 13\,847 & 17\,315 & 94\,452 & 47\,205 & 178\,002 & 178\,002 & 19\,012 & 221\,837 \\
%     Thailand & 8\,983 & 15\,037 & 58\,398 & 29\,140 & 125\,405 & 125\,405 & 11\,512 & 155\,671 \\
%     Nigeria & 6\,073 & 6\,368 & 42\,080 & 21\,017 & 77\,514 & 77\,514 & 8\,352 & 93\,702 \\
%     Malaysia & 6\,008 & 9\,788 & 38\,208 & 19\,058 & 80\,754 & 80\,754 & 7\,516 & 98\,624 \\
%     Vietnam & 5\,048 & 5\,744 & 37\,035 & 18\,492 & 58\,661 & 58\,661 & 7\,345 & 71\,855 \\
%     Bangladesh & 5\,023 & 9\,236 & 29\,253 & 14\,599 & 62\,839 & 62\,839 & 5\,768 & 77\,646 \\
%     Pakistan & 4\,761 & 6\,973 & 38\,005 & 18\,961 & 77\,271 & 77\,271 & 7\,516 & 98\,251 \\
%     Sri Lanka & 1\,977 & 2\,651 & 14\,643 & 7\,306 & 29\,512 & 29\,512 & 2\,857 & 37\,128 \\
%     Saudi Arabia & 1\,874 & 2\,292 & 17\,759 & 8\,868 & 35\,921 & 35\,921 & 3\,547 & 45\,309 \\
%     Kenya & 1\,769 & 2\,763 & 17\,251 & 8\,610 & 36\,397 & 36\,397 & 3\,537 & 46\,305 \\
%     Ethiopia & 1\,399 & 2\,163 & 14\,244 & 7\,112 & 30\,317 & 30\,317 & 2\,920 & 38\,791 \\
%     Mongolia & 1\,032 & 1\,306 & 12\,482 & 6\,237 & 23\,611 & 23\,611 & 2\,452 & 29\,912 \\
%     Tanzania & 969 & 1\,454 & 11\,966 & 5\,983 & 26\,440 & 26\,440 & 2\,406 & 34\,260 \\
%     Rwanda & 773 & 1\,393 & 7\,332 & 3\,665 & 15\,711 & 15\,711 & 1\,469 & 19\,977 \\
%     Mexico & 20\,622 & 29\,724 & 184\,998 & 92\,497 & 363\,479 & 363\,479 & 37\,179 & 450\,496 \\
%     Egypt & 6\,561 & 9\,596 & 63\,237 & 31\,616 & 131\,069 & 131\,069 & 12\,692 & 173\,320 \\
%     Singapore & 2\,589 & 4\,298 & 23\,619 & 11\,811 & 49\,920 & 49\,920 & 4\,858 & 70\,143 \\
%     \midrule
%     \textbf{Total} & 3\,044\,895 & 2\,879\,840 & 15\,871\,990 & 7\,933\,015 & 21\,986\,501 & 14\,105\,480 & 5\,457\,881 & 17\,906\,439 \\
%     \bottomrule
%   \end{tabular}%
%   }
%     \caption{Comprehensive data statistics across 42 cultural regions: raw VQA extraction counts (entities, images, open-ended questions, multiple-choice questions) and final sample counts after temperature-based region sampling with hybrid sampling strategy.}
%     \label{tab:region_data_full_condensed}
% \end{table*}


% \begin{table*}[t]
%   \centering
%   \scriptsize
%   \setlength{\tabcolsep}{3pt}
%   \resizebox{\textwidth}{!}{%
%   \begin{tabular}{l*{6}{r}}
%     \toprule
%     \multirow{2}{*}{\textbf{Region}} 
%       & \multirow{2}{*}{\textbf{# Samples}} 
%       & \multicolumn{4}{c}{\textbf{Region Sampling}} 
%       & \multirow{2}{*}{\textbf{Total}} \\
%       \cmidrule(lr){3-6}
%     & & \textbf{OE Available} & \textbf{OE Sampled} & \textbf{MCQ Available} & \textbf{MCQ Sampled} & \\
%     \midrule
%     Germany         & 2\,766\,801 & 1\,506\,700 &   651\,674 &   25\,757 &   25\,757 &   677\,431 \\
%     France          & 2\,697\,046 & 1\,436\,143 &   641\,338 &  236\,880 &  208\,244 &   849\,582 \\
%     United Kingdom & 2\,143\,875 & 1\,319\,729 &   623\,519 &   64\,048 &   64\,048 &   687\,567 \\
%     Czechia         &   969\,181 &   679\,129 &   499\,657 &  188\,017 &  188\,017 &   687\,674 \\
%     Spain           & 1\,500\,771 &   908\,936 &   550\,638 &  380\,167 &  243\,812 &   794\,450 \\
%     Italy           & 1\,763\,270 & 1\,324\,123 &   624\,210 &   46\,855 &   46\,855 &   671\,065 \\
%     Poland          &   919\,493 &   529\,738 &   459\,948 &   11\,099 &   11\,099 &   471\,047 \\
%     Russia          &   848\,672 &   628\,718 &   486\,975 &  528\,649 &  272\,136 &   759\,111 \\
%     Japan           & 1\,213\,376 &   800\,123 &   527\,724 &  426\,350 &  253\,310 &   781\,034 \\
%     Netherlands     &   375\,073 &   225\,701 &   225\,701 &   96\,070 &   96\,070 &   321\,771 \\
%     Ukraine         &   562\,642 &   421\,134 &   421\,134 &  270\,474 &  217\,656 &   638\,790 \\
%     Brazil          &   648\,473 &   479\,452 &   444\,907 &   80\,265 &   80\,265 &   525\,172 \\
%     China           &   469\,734 &   365\,867 &   365\,867 &  103\,545 &  103\,545 &   469\,412 \\
%     India           &   717\,392 &   542\,900 &   463\,726 &   72\,361 &   72\,361 &   536\,087 \\
%     Norway          &   382\,252 &   273\,705 &   273\,705 &  106\,083 &  106\,083 &   379\,788 \\
%     Portugal        &   237\,161 &   162\,195 &   162\,195 &  654\,153 &  292\,161 &   454\,356 \\
%     Israel          &   289\,501 &   234\,144 &   234\,144 &  431\,828 &  254\,390 &   488\,534 \\
%     Romania         &   287\,120 &   194\,969 &   194\,969 &   14\,660 &   14\,660 &   209\,629 \\
%     Indonesia       &   257\,335 &   149\,295 &   149\,295 &   31\,457 &   31\,457 &   180\,752 \\
%     Turkey          &   256\,807 &   184\,007 &   184\,007 &  120\,705 &  120\,705 &   304\,712 \\
%     South Korea    &   209\,979 &   123\,627 &   123\,627 &    8\,769 &    8\,769 &   132\,396 \\
%     Iran            &   252\,409 &   195\,017 &   195\,017 &  114\,628 &  114\,628 &   309\,645 \\
%     Greece          &   250\,547 &   173\,277 &   173\,277 &   26\,041 &   26\,041 &   199\,318 \\
%     Taiwan          &   166\,456 &   142\,812 &   142\,812 &  118\,472 &  118\,472 &   261\,284 \\
%     Ireland         &   185\,142 &   146\,718 &   146\,718 &   29\,638 &   29\,638 &   176\,356 \\
%     Bulgaria        &   177\,919 &   129\,713 &   129\,713 &  328\,193 &  232\,152 &   361\,865 \\
%     Thailand        &   125\,380 &   101\,179 &   101\,179 &   93\,724 &   93\,724 &   194\,903 \\
%     Nigeria         &    77\,475 &    53\,507 &    53\,507 &  104\,136 &  104\,136 &   157\,643 \\
%     Malaysia        &    80\,695 &    64\,338 &    64\,338 &  311\,499 &  228\,147 &   292\,485 \\
%     Vietnam         &    58\,623 &    43\,716 &    43\,716 &    5\,830 &    5\,830 &    49\,546 \\
%     Bangladesh      &    62\,795 &    51\,163 &    51\,163 &   13\,379 &   13\,379 &    64\,542 \\
%     Pakistan        &    77\,228 &    60\,007 &    60\,007 &   17\,766 &   17\,766 &    77\,773 \\
%     Sri\_Lanka      &    29\,489 &    22\,177 &    22\,177 &   65\,269 &   65\,269 &    87\,446 \\
%     Saudi Arabia   &    35\,900 &    27\,181 &    27\,181 &  546\,246 &  275\,122 &   302\,303 \\
%     Kenya           &    36\,395 &    29\,171 &    29\,171 &   10\,913 &   10\,913 &    40\,084 \\
%     Ethiopia        &    30\,259 &    23\,978 &    23\,978 &   70\,111 &   70\,111 &    94\,089 \\
%     Mongolia        &    23\,611 &    16\,436 &    16\,436 &   11\,611 &   11\,611 &    28\,047 \\
%     Tanzania        &    26\,426 &    17\,771 &    17\,771 &   49\,997 &   49\,997 &    67\,768 \\
%     Rwanda          &    15\,711 &    11\,868 &    11\,868 &   99\,449 &   99\,449 &   111\,317 \\
%     Singapore       &    49\,920 &    38\,919 &    38\,919 &  207\,452 &  199\,236 &   238\,155 \\
%     Mexico          &   363\,365 &   267\,570 &   267\,570 &  469\,507 &  261\,583 &   529\,153 \\
%     Egypt           &   131\,042 &   100\,830 &   100\,830 &   21\,882 &   21\,882 &   122\,712 \\
%     \midrule
%     \textbf{Total}  &21\,772\,741 &14\,207\,683 &10\,026\,308 & 6\,613\,935 & 4\,760\,486 &14\,786\,794 \\
%     \bottomrule
%   \end{tabular}%
%   }
%     \caption{Quality-filtered dataset statistics by region: comparison of available samples versus sampled data for open-ended (OE) and multiple-choice questions (MCQs) after applying quality filtering and conservative temperature sampling (3.0 for regions, 1.5 for languages).}
%     \label{tab:region_sampling_filtered}
% \end{table*}



==> latex/tables/xm100.tex <==
% \begin{table}[!h]
% \centering
% \resizebox{0.95\textwidth}{!}{%
% \begin{tabular}{l|cccccccc}
% \toprule
% \textbf{Models} & \textbf{English} & \textbf{Multi} & \textbf{Arabic} & \textbf{Bengali} & \textbf{Czech} & \textbf{Danish} & \textbf{German} & \textbf{Greek} \\
% \midrule
% Llava-Next-7B          & 92.4         & 15.5       & 5.0        & 0.0        & 27.3       & 22.6       & 23.8       & 2.4        \\
% Molmo-7B-D             & 4.7          & 6.0        & 5.5        & 2.7        & 2.8        & 7.6        & 9.5        & 2.6        \\
% Llama3.2-11B           & 23.1         & 5.8        & 0.0        & 0.0        & 0.2        & 15.3       & 4.4        & 0.5        \\
% PaliGemma-3B           & 24.7         & 0.6        & 0.0        & 0.0        & 0.6        & 1.0        & 3.1        & 0.0        \\
% mBLIP mT0-XL           & 101.0        & 6.8        & 7.7        & 2.7        & 11.2       & 6.9        & 5.8        & 7.7        \\
% AyaVision-8B           & 10.3         & 10.0       & 7.8        & 7.7        & 9.3        & 7.9        & 11.7       & 6.0        \\
% Pangea-7B              & 93.2         & 29.7       & 39.6       & 25.1       & 27.5       & 32.4       & 42.7       & 11.9       \\
% \model       & 90.8         & 36.9       & 41.2       & 29.6       & 39.4       & 30.9       & 51.7       & 21.3       \\
% \midrule
% \textbf{Models} & \textbf{Spanish} & \textbf{Persian} & \textbf{Finnish} & \textbf{Filipino} & \textbf{French} & \textbf{Hebrew} & \textbf{Hindi} & \textbf{Croatian} \\
% \midrule
% Llava-Next-7B          & 59.6         & 4.8        & 9.3        & 6.2        & 61.9       & 3.0        & 3.9        & 7.4        \\
% Molmo-7B-D             & 8.3          & 7.2        & 2.0        & 2.4        & 18.5       & 10.6       & 2.5        & 2.2        \\
% Llama3.2-11B           & 14.9         & 0.0        & 2.3        & 11.0       & 20.0       & 0.0        & 0.0        & 0.6        \\
% PaliGemma-3B           & 0.5          & 0.0        & 0.0        & 0.1        & 1.3        & 0.0        & 0.0        & 0.3        \\
% mBLIP mT0-XL           & 19.0         & 11.5       & 4.7        & 5.9        & 10.9       & 9.4        & 2.0        & 2.2        \\
% AyaVision-8B           & 14.5         & 15.5       & 2.0        & 2.5        & 15.1       & 20.4       & 3.5        & 4.3        \\
% Pangea-7B              & 96.5         & 34.7       & 8.6        & 13.8       & 71.0       & 33.3       & 30.4       & 13.9       \\
% \model       & 82.9         & 38.5       & 3.5        & 10.0       & 77.7       & 42.5       & 28.4       & 14.2       \\
% \midrule
% \textbf{Models} & \textbf{Hungarian} & \textbf{Indonesian} & \textbf{Italian} & \textbf{Japanese} & \textbf{Korean} & \textbf{Maori} & \textbf{Dutch} & \textbf{Norwegian} \\
% \midrule
% Llava-Next-7B          & 16.7         & 20.5       & 36.3       & 1.1        & 10.1       & 2.4        & 50.7       & 27.2       \\
% Molmo-7B-D             & 1.5          & 25.8       & 12.5       & 1.2        & 4.5        & 1.0        & 8.5        & 5.6        \\
% Llama3.2-11B           & 18.3         & 1.4        & 22.1       & 0.0        & 0.0        & 2.3        & 35.6       & 0.6        \\
% PaliGemma-3B           & 0.4          & 0.3        & 0.4        & 0.0        & 0.0        & 2.3        & 3.1        & 0.5        \\
% mBLIP mT0-XL           & 7.6          & 8.9        & 4.8        & 1.1        & 4.5        & 4.2        & 11.1       & 7.2        \\
% AyaVision-8B           & 2.5          & 27.0       & 19.0       & 3.6        & 11.4       & 0.2        & 12.0       & 5.9        \\
% Pangea-7B              & 9.6          & 64.6       & 54.4       & 0.5        & 20.4       & 0.6        & 56.3       & 53.3       \\
% \model       & 6.1          & 57.7       & 58.3       & 0.7        & 23.1       & 0.6        & 63.6       & 58.3       \\
% \midrule
% \textbf{Models} & \textbf{Polish} & \textbf{Portuguese} & \textbf{Quechua} & \textbf{Romanian} & \textbf{Russian} & \textbf{Swedish} & \textbf{Swahili} & \textbf{Telugu} \\
% \midrule
% Llava-Next-7B          & 21.8         & 48.2       & 0.0        & 14.9       & 20.2       & 31.9       & 0.6        & 0.0        \\
% Molmo-7B-D             & 3.7          & 8.5        & 0.2        & 5.4        & 12.5       & 4.9        & 0.0        & 0.4        \\
% Llama3.2-11B           & 1.1          & 24.5       & 0.0        & 10.5       & 0.5        & 9.1        & 6.5        & 0.0        \\
% PaliGemma-3B           & 0.6          & 2.8        & 0.1        & 1.1        & 0.0        & 2.0        & 0.0        & 0.0        \\
% mBLIP mT0-XL           & 11.2         & 10.8       & 0.6        & 4.3        & 7.9        & 11.0       & 7.5        & 7.4        \\
% AyaVision-8B           & 13.2         & 11.5       & 0.2        & 23.1       & 21.6       & 6.0        & 1.4        & 3.6        \\
% Pangea-7B              & 33.8         & 82.6       & 0.0        & 41.7       & 62.0       & 30.8       & 45.8       & 0.0        \\
% \model       & 48.0         & 87.5       & 0.8        & 43.4       & 66.1       & 23.0       & 46.8       & 27.6       \\
% \midrule\midrule
% \textbf{Models} & \textbf{Thai} & \textbf{Turkish} & \textbf{Ukrainian} & \textbf{Vietnamese} & \textbf{Chinese} &  &  &  \\
% \midrule
% Llava-Next-7B          & 0.0          & 0.0        & 0.1         & 0.0          & 1.1         &            &            &            \\
% Molmo-7B-D             & 0.0          & 3.8        & 3.8         & 20.5         & 0.0         &            &            &            \\
% Llama3.2-11B           & 0.0          & 0.0        & 0.0         & 0.0          & 0.0         &            &            &            \\
% PaliGemma-3B           & 0.9          & 0.0        & 0.0         & 0.4          & 0.0         &            &            &            \\
% mBLIP mT0-XL           & 0.0          & 9.9        & 4.0         & 6.6          & 0.0         &            &            &            \\
% AyaVision-8B           & 0.0          & 14.7       & 14.9       & 25.2       & 4.0       &            &            &            \\
% Pangea-7B              & 0.0          & 0.0        & 0.0         & 0.0          & 0.9         &            &            &            \\
% \model       & 0.0          & 44.3       & 39.9       & 84.1       & 0.5       &            &            &            \\
% \bottomrule
% \end{tabular}%
% }
% \caption{Comparison of models on the XM100 dataset across different languages.}
% \label{tab:breakdown_XM100}
% \end{table}



% \begin{table*}[t]
%   \centering
%   \scriptsize
%   \captionsetup[subtable]{skip=1ex}

%   % Languages 1–12
%   \begin{subtable}{\textwidth}
%     \centering
%     \setlength{\tabcolsep}{3pt}
%     \begin{adjustbox}{width=\textwidth}
%       \begin{tabular}{l@{}*{12}{>{\centering\arraybackslash}p{1.2cm}@{}}}
%         \toprule
%         Models & \rotatebox{90}{English} & \rotatebox{90}{Multi} & \rotatebox{90}{Arabic} & \rotatebox{90}{Bengali} & \rotatebox{90}{Czech} & \rotatebox{90}{Danish} & \rotatebox{90}{German} & \rotatebox{90}{Greek} & \rotatebox{90}{Spanish} & \rotatebox{90}{Persian} & \rotatebox{90}{Finnish} & \rotatebox{90}{Filipino} \\
%         \midrule
%         Llava-Next-7B    & 92.4 & 15.5 & 5.0 & 0.0 & 27.3 & 22.6 & 23.8 & 2.4 & 59.6 & 4.8 & 9.3 & 6.2 \\
%         Molmo-7B-D       & 4.7  & 6.0  & 5.5 & 2.7 & 2.8  & 7.6  & 9.5  & 2.6 & 8.3  & 7.2 & 2.0 & 2.4 \\
%         Llama3.2-11B     & 23.1 & 5.8  & 0.0 & 0.0 & 0.2  & 15.3 & 4.4  & 0.5 & 14.9 & 0.0 & 2.3 & 11.0 \\
%         PaliGemma-3B     & 24.7 & 0.6  & 0.0 & 0.0 & 0.6  & 1.0  & 3.1  & 0.0 & 0.5  & 0.0 & 0.0 & 0.1 \\
%         mBLIP mT0-XL     & 101.0& 6.8  & 7.7 & 2.7 & 11.2 & 6.9  & 5.8  & 7.7 & 19.0 & 11.5& 4.7 & 5.9 \\
%         AyaVision-8B     & 10.3 & 10.0 & 7.8 & 7.7 & 9.3  & 7.9  & 11.7 & 6.0 & 14.5 & 15.5& 2.0 & 2.5 \\
%         Pangea-7B        & 93.2 & 29.7 & 39.6& 25.1& 27.5 & 32.4 & 42.7 & 11.9& 96.5 & 34.7& 8.6 & 13.8 \\
%         \model & 90.8 & 36.9 & 41.2& 29.6& 39.4 & 30.9 & 51.7 & 21.3& 82.9 & 38.5& 3.5 & 10.0 \\
%         \bottomrule
%       \end{tabular}
%     \end{adjustbox}
%     \caption{Languages 1--12}
%   \end{subtable}

%   \bigskip

%   % Languages 13–25
%   \begin{subtable}{\textwidth}
%     \centering
%     \setlength{\tabcolsep}{2.5pt}
%     \begin{adjustbox}{width=\textwidth}
%       \begin{tabular}{l@{}*{13}{>{\centering\arraybackslash}p{1.15cm}@{}}}
%         \toprule
%         Models & \rotatebox{90}{French} & \rotatebox{90}{Hebrew} & \rotatebox{90}{Hindi} & \rotatebox{90}{Croatian} & \rotatebox{90}{Hungarian} & \rotatebox{90}{Indonesian} & \rotatebox{90}{Italian} & \rotatebox{90}{Japanese} & \rotatebox{90}{Korean} & \rotatebox{90}{Maori} & \rotatebox{90}{Dutch} & \rotatebox{90}{Norwegian} & \rotatebox{90}{Polish} \\
%         \midrule
%         Llava-Next-7B    & 61.9 & 3.0  & 3.9  & 7.4  & 16.7  & 20.5      & 36.3    & 1.1      & 10.1   & 2.4     & 50.7   & 27.2      & 21.8       \\
%         Molmo-7B-D       & 18.5 & 10.6 & 2.5  & 2.2  & 1.5   & 25.8      & 12.5    & 1.2      & 4.5    & 1.0     & 8.5    & 5.6       & 3.7        \\
%         Llama3.2-11B     & 20.0 & 0.0  & 0.0  & 0.6  & 18.3  & 1.4       & 22.1    & 0.0      & 0.0    & 2.3     & 35.6   & 0.6       & 1.1        \\
%         PaliGemma-3B     & 1.3  & 0.0  & 0.0  & 0.3  & 0.4   & 0.3       & 0.4     & 0.0      & 0.0    & 2.3     & 3.1    & 0.5       & 0.6        \\
%         mBLIP mT0-XL     & 10.9 & 9.4  & 2.0  & 2.2  & 7.6   & 8.9       & 4.8     & 1.1      & 4.5    & 4.2     & 11.1   & 7.2       & 11.2       \\
%         AyaVision-8B     & 15.1 & 20.4 & 3.5  & 4.3  & 2.5   & 27.0      & 19.0    & 3.6      & 11.4   & 0.2     & 12.0   & 5.9       & 13.2       \\
%         Pangea-7B        & 71.0 & 33.3 & 30.4 & 13.9 & 9.6   & 64.6      & 54.4    & 0.5      & 20.4   & 0.6     & 56.3   & 53.3      & 33.8       \\
%         \model & 77.7 & 42.5 & 28.4 & 14.2 & 6.1   & 57.7      & 58.3    & 0.7      & 23.1   & 0.6     & 63.6   & 58.3      & 48.0       \\
%         \bottomrule
%       \end{tabular}
%     \end{adjustbox}
%     \caption{Languages 13--25}
%   \end{subtable}

%   \bigskip

%   % Languages 26–37
%   \begin{subtable}{\textwidth}
%     \centering
%     \setlength{\tabcolsep}{3pt}
%     \begin{adjustbox}{width=\textwidth}
%       \begin{tabular}{l@{}*{12}{>{\centering\arraybackslash}p{1.2cm}@{}}}
%         \toprule
%         Models & \rotatebox{90}{Portuguese} & \rotatebox{90}{Quechua} & \rotatebox{90}{Romanian} & \rotatebox{90}{Russian} & \rotatebox{90}{Swedish} & \rotatebox{90}{Swahili} & \rotatebox{90}{Telugu} & \rotatebox{90}{Thai} & \rotatebox{90}{Turkish} & \rotatebox{90}{Ukrainian} & \rotatebox{90}{Vietnamese} & \rotatebox{90}{Chinese} \\
%         \midrule
%         Llava-Next-7B    & 48.2 & 0.0  & 14.9 & 20.2 & 31.9 & 0.6  & 0.0  & 0.0 & 0.0  & 0.1 & 0.0  & 1.1  \\
%         Molmo-7B-D       & 8.5  & 0.2  & 5.4  & 12.5 & 4.9  & 0.0  & 0.4  & 0.0 & 3.8  & 3.8 & 20.5 & 0.0  \\
%         Llama3.2-11B     & 24.5 & 0.0  & 10.5 & 0.5  & 9.1  & 6.5  & 0.0  & 0.0 & 0.0  & 0.0 & 0.0  & 0.0  \\
%         PaliGemma-3B     & 2.8  & 0.1  & 1.1  & 0.0  & 2.0  & 0.0  & 0.0  & 0.9 & 0.0  & 0.0 & 0.4  & 0.0  \\
%         mBLIP mT0-XL     & 10.8 & 0.6  & 4.3  & 7.9  & 11.0 & 7.5  & 7.4  & 0.0 & 9.9  & 4.0 & 6.6  & 0.0  \\
%         AyaVision-8B     & 11.5 & 0.2  & 23.1 & 21.6 & 6.0  & 1.4  & 3.6  & 0.0 & 14.7 & 14.9& 25.2 & 4.0  \\
%         Pangea-7B        & 82.6 & 0.0  & 41.7 & 62.0 & 30.8 & 45.8 & 0.0  & 0.0 & 0.0  & 0.0 & 0.0  & 0.9  \\
%         \model & 87.5 & 0.8  & 43.4 & 66.1 & 23.0 & 46.8 & 27.6 & 0.0 & 44.3 & 39.9& 84.1 & 0.5  \\
%         \bottomrule
%       \end{tabular}
%     \end{adjustbox}
%     \caption{Languages 26--37}
%   \end{subtable}

%   \caption{XM100 benchmark performance (\%) of eight multimodal models across 37 languages.}
%   \label{tab:breakdown_XM100_simple}
% \end{table*}

